Learning the Topology and Behavior of Discrete Dynamical Systems

Discrete dynamical systems are commonly used to model the spread of contagions on real-world networks. Under the PAC framework, existing research has studied the problem of learning the behavior of a system, assuming that the underlying network is known. In this work, we focus on a more challenging setting: to learn both the behavior and the underlying topology of a black-box system. We show that, in general, this learning problem is computationally intractable. On the positive side, we present efficient learning methods under the PAC model when the underlying graph of the dynamical system belongs to some classes. Further, we examine a relaxed setting where the topology of an unknown system is partially observed. For this case, we develop an efficient PAC learner to infer the system and establish the sample complexity. Lastly, we present a formal analysis of the expressive power of the hypothesis class of dynamical systems where both the topology and behavior are unknown, using the well-known formalism of the Natarajan dimension. Our results provide a theoretical foundation for learning both the behavior and topology of discrete dynamical systems.

==> tex/titlepage.tex <==
% !TEX root = ./main.tex

\begin{titlepage}

{

%\center{\textcolor{red}{For Evaluation By PKDD Only --- Not for Public Use/Consumption\\
%To be Released at a Later Date}}

\normalsize
\rightline{\bf NDSSL Technical Report 2017-1035}
%\medskip
\vspace{0.2in}
\normalsize{\hfill{Sept. 17, 2017}}

\vspace{0.05in}
\noindent\begin{tabular}{r|p{0.75\textwidth}}
\rule[0.25in]{0pt}{0pt} & \\
Title:&\normalsize{Learning and Inference in Networked Social Systems -- Part 2:} \\
      &\normalsize{Deterministic Query Generation Methods} \\
\rule[0.5in]{0pt}{0pt} & \\
Authors: &
\small{
Abhijin Adiga\newline
Christopher J. Kuhlman\newline
Madhav V. Marathe\newline
S. S. Ravi\newline
Daniel J. Rosenkrantz\newline
Richard E. Stearns}\\

%\institute{
%Virginia Bioinformatics Institute, Virginia Tech, Blacksburg, 
%VA 24061, USA.
%Email:~ \texttt{\{ckuhlman,akumar,mmarathe\}@vbi.vt.edu} \\ \and
%Computer Science Department, University at Albany -- SUNY, 
%Albany, NY 12222, USA.
%Email:~ \texttt{\{ravi,djr\}@cs.albany.edu}
%}

\rule[0.25in]{0pt}{0pt} & \\
Contact: &
\small{Madhav V. Marathe\newline
 Email: {\tt mmarathe@bi.vt.edu} \newline
 Tel.: +1 540 231 8832\newline
 Fax: +1 540 231 2891} \\
\rule[0.25in]{0pt}{0pt} & \\

%To Appear In: &
%%Submitted To: &
%\small{The 10th IEEE International Conference on e-Science (eScience 2014)}\\
%%\small{}\\


\rule[0.25in]{0pt}{0pt} & \\
Acknowledgments: & \small{
We convey our special thanks to 
Noshir Contractor (Northwestern University),
Joshua Epstein (New York University),
Brian Goode (Virginia Tech),
Michael Macy (Cornell University), 
Naren Ramakrishnan (Virginia Tech) and
Nathan Self (Virginia Tech)
for discussions on topics related to the paper.
This work has been partially supported by
DARPA Cooperative Agreement D17AC00003 (NGS2),
DTRA CNIMS (Contract HDTRA1-11-D-0016-0001),
NSF DIBBS Grant ACI-1443054 and
NSF BIG DATA Grant IIS-1633028.
The U.S. Government is authorized to reproduce and
distribute reprints for Governmental purposes notwithstanding
any copyright annotation thereon.

\bigskip

\noindent
\textbf{Disclaimer:}~ The views and conclusions contained herein are those 
of the authors and should
not be interpreted as necessarily representing the 
official policies or endorsements, either expressed
or implied, of DARPA or the U.S. Government.
} \\
\rule[0.25in]{0pt}{0pt} & \\
\end{tabular}

\vfill

\rightline{\makebox[3.5in][l]{\vbox{\small
\noindent Network Dynamics and Simulation Science Laboratory\\
Biocomplexity Institute of Virginia Tech\\
Virginia Polytechnic Institute and State University\\
%%and\\
%%Computer Science Department, University at Albany -- SUNY
}}}

%\noindent\includegraphics[width=\textwidth]{VBI_VT_Logo.eps}
\title{}
\author{}
\date{}

%\textcolor{red}{For Evaluation By PKDD Only --- Not for Public Use/Consumption}

}

\bigskip\bigskip

\begin{center}
\fbox{\fbox{\Large{\textbf{Preliminary Version:~ Please Do Not Distribute}}}}
\end{center}

\thispagestyle{empty}

\end{titlepage}

